HappyQuokka System for ICASSP 2023 Auditory EEG Challenge

This report describes our submission to Task 2 of the Auditory EEG Decoding Challenge at ICASSP 2023 Signal Processing Grand Challenge (SPGC). Task 2 is a regression problem that focuses on reconstructing a speech envelope from an EEG signal. For the task, we propose a pre-layer normalized feed-forward transformer (FFT) architecture. For within-subjects generation, we additionally utilize an auxiliary global conditioner which provides our model with additional information about seen individuals. Experimental results show that our proposed method outperforms the VLAAI baseline and all other submitted systems. Notably, it demonstrates significant improvements on the within-subjects task, likely thanks to our use of the auxiliary global conditioner. In terms of evaluation metrics set by the challenge, we obtain Pearson correlation values of 0.1895 0.0869 for the within-subjects generation test and 0.0976 0.0444 for the heldout-subjects test. We release the training code for our model online.

==> instructions.tex <==
Hi all,
please follow the below ICASSP instructions for submission of the 2-page paper:


1)      Use the same template for regular ICASSP papers, but with a page length of max 2 pages (instead of 4+1). This includes everything (title, abstract, intro, references, and possible figures and tables).

2)      The abstract and introduction must clearly mention that this work is done in the context of an  “ICASSP Signal Processing Grand Challenge“ ( +include (a) official challenge name, (b) the year of the challenge, and if applicable (c) the edition number if this is not the first edition of the challenge)

3)      The paper is free format, but must not exceed 2 pages (including references), and should contain an abstract and (brief) introduction.

4)      The introduction should at least contain:

a.       a brief description of the scope of the challenge (+ challenge name, see above)

b.       a brief description of your proposed solution (its main ingredients)

c.       the quantitative results you obtained on the challenge’s evaluation metrics.   

It is not necessary to exhaustively describe prior art in the introduction. However, standard citation rules remain applicable. E.g. if your solution is inspired by (or uses) existing work, cite it properly.

5)      In the main text, focus on the conceptual implementation/innovation, and a high-level description of the proposed solution.

6)      In general: make the paper as self-contained as possible. Yet, keep in mind that you still have the opportunity to submit a full journal paper to OJSP if you feel your methodology is sufficiently innovative to be published as a journal paper.
